Look here! A parametric learning based approach to redirect visual attention

Across photography, marketing, and website design, being able to direct the viewer's attention is a powerful tool. Motivated by professional workflows, we introduce an automatic method to make an image region more attention-capturing via subtle image edits that maintain realism and fidelity to the original. From an input image and a user-provided mask, our GazeShiftNet model predicts a distinct set of global parametric transformations to be applied to the foreground and background image regions separately. We present the results of quantitative and qualitative experiments that demonstrate improvements over prior state-of-the-art. In contrast to existing attention shifting algorithms, our global parametric approach better preserves image semantics and avoids typical generative artifacts. Our edits enable inference at interactive rates on any image size, and easily generalize to videos. Extensions of our model allow for multi-style edits and the ability to both increase and attenuate attention in an image region. Furthermore, users can customize the edited images by dialing the edits up or down via interpolations in parameter space. This paper presents a practical tool that can simplify future image editing pipelines.

==> README <==
==========================================================================

The `caption' package bundle
Release 2020-07-20
Copyright (C) 1994-2020 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  https://gitlab.com/axelsommerfeldt/caption

If you need help for installation please visit:
  https://texfaq.org/FAQ-inst-miktexstar
  https://texfaq.org/FAQ-installthings
  https://texfaq.org/FAQ-privinst

If you need help using these packages please visit:
  https://latex.org/forum/
  https://tex.stackexchange.com/
  https://golatex.de/               (German)
  https://texwelt.de/               (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  https://gitlab.com/axelsommerfeldt/caption/issues (preferred)
or send an e-mail to
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.4 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.2 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.3 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

Note: The `newfloat' package was removed from this package bundle and was
uploaded to CTAN as stand-alone package.

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)

